Confessions of a Masked MDP

In reinforcement learning, one presumes the action set to be known ahead of time, and, thus, one must know if any state-action pairs are not permissible ahead of computations. In some applications, determining this action mask is the main computational bottleneck. Isolating this problem to highlight its core properties, we study how to combine the search for an optimal policy with the learning of the mask itself, under a linear MDP model in which each attempted action reveals the exact value of a linear score determining its validity. In this framework, we first construct an algorithm based on deterministic optimistic optimization and show that it is minimax optimal, which we show is also computationally efficient. However, it is sub-optimal on non-degenerate instances, as we show. We propose an alternative, which is also computationally efficient, which plans its exploration strategy. This algorithm admits a formal interpretation as an analogue of information-directed-sampling for deterministic feedback, which may be of independent interest. Finally, we study an application of this framework to transfer learning, where the invalid action set changes over time.

==> macro_table.tex <==

\RequirePackage{array}
\RequirePackage{booktabs}
\RequirePackage{longtable}

\providecommand{\macrorow}[3]{%
  #1 & \texttt{\detokenize{#2}} & \ensuremath{#3} \\
}

\providecommand{\macrotablesection}[1]{%
  \addlinespace[0.5em]
  \multicolumn{3}{l}{\textbf{#1}} \\
  \addlinespace[0.2em]
}

\providecommand{\printmacrotable}{%
  \begingroup
  \small
  \setlength{\LTleft}{0pt}
  \setlength{\LTright}{0pt}
  \setlength{\tabcolsep}{6pt}
  \renewcommand{\arraystretch}{1.2}
  \begin{longtable}{%
    >{\raggedright\arraybackslash}p{0.37\textwidth}
    >{\raggedright\arraybackslash}p{0.35\textwidth}
    >{\centering\arraybackslash}p{0.18\textwidth}}
    \caption{Shared LaTeX macros defined in \texttt{united\_macros.tex}.}
    \label{tab:shared-macros}\\
    \toprule
    \textbf{Concept} & \textbf{Macro} & \textbf{Appearance} \\
    \midrule
    \endfirsthead

    \multicolumn{3}{c}{\tablename~\thetable\ (continued)} \\
    \toprule
    \textbf{Concept} & \textbf{Macro} & \textbf{Appearance} \\
    \midrule
    \endhead

    \midrule
    \multicolumn{3}{r}{Continued on next page} \\
    \endfoot

    \bottomrule
    \endlastfoot

    \macrotablesection{Base MDP}
    \macrorow{Markov decision process}{\MDP}{\MDP}
    \macrorow{Base/source MDP}{\baseMDP}{\baseMDP}
    \macrorow{Task-indexed MDP}{\taskMDP{\episode}}{\taskMDP{\episode}}
    \macrorow{State space}{\statespace}{\statespace}
    \macrorow{State}{\state}{\state}
    \macrorow{Augmented state space}{\augstatespace}{\augstatespace}
    \macrorow{Action space}{\actionspace}{\actionspace}
    \macrorow{Action}{\action}{\action}
    \macrorow{Transition kernel}{\transition}{\transition}
    \macrorow{Expected reward}{\reward}{\reward}
    \macrorow{Random reward}{\randreward}{\randreward}
    \macrorow{Horizon}{\horizon}{\horizon}
    \macrorow{Policy}{\policy}{\policy}
    \macrorow{Regret}{\regret}{\regret}
    \macrorow{Cemetery state}{\cemetery}{\cemetery}

    \macrotablesection{Linear model and masks}
    \macrorow{Feature map}{\feature}{\feature}
    \macrorow{Feature-map capital}{\Feature}{\Feature}
    \macrorow{Transition feature}{\transitionfeature}{\transitionfeature}
    \macrorow{Reward parameter}{\rewardfeature}{\rewardfeature}
    \macrorow{Masked feature}{\featuremask}{\featuremask}
    \macrorow{Feature space}{\featurespace}{\featurespace}
    \macrorow{Mask}{\mask}{\mask}
    \macrorow{Mask parameter}{\maskpar}{\maskpar}
    \macrorow{Mask sequence}{\masksequence}{\masksequence}
    \macrorow{Mask class}{\maskclass}{\maskclass}
    \macrorow{Classifier}{\classifier}{\classifier}
    \macrorow{Hypothesis class}{\hypclass}{\hypclass}
    \macrorow{Calligraphic H helper}{\Hc}{\Hc}
    \macrorow{Gap, margin, or one-step gap}{\gap}{\gap}
    \macrorow{Diameter}{\diameter}{\diameter}

    \macrotablesection{Knowledge states and passive planner}
    \macrorow{Initial-state law}{\startlaw}{\startlaw}
    \macrorow{State--action pair}{\pair}{\pair}
    \macrorow{State--action pair space}{\pairspace}{\pairspace}
    \macrorow{Feature of a pair}{\pairfeature{\pair}}{\pairfeature{\pair}}
    \macrorow{Mask-indexed MDP}{\maskMDP{\maskpar}}{\maskMDP{\maskpar}}
    \macrorow{Valid-action set}{\validactions{\maskpar}}{\validactions{\maskpar}}
    \macrorow{Masked reward}{\maskedreward{\maskpar}}{\maskedreward{\maskpar}}
    \macrorow{Masked transition}{\maskedtransition{\maskpar}}{\maskedtransition{\maskpar}}
    \macrorow{First invalid step}{\firstinvalid}{\firstinvalid}
    \macrorow{Reveal set}{\revealset}{\revealset}
    \macrorow{Episode cost}{\episodecost}{\episodecost}
    \macrorow{Version/knowledge state}{\versionstate}{\versionstate}
    \macrorow{Observed-pair multiset}{\observedpairs}{\observedpairs}
    \macrorow{Observed span}{\observedspan}{\observedspan}
    \macrorow{Decided directions}{\decideddirections}{\decideddirections}
    \macrorow{Linear span operator}{\spn}{\spn}
    \macrorow{Lower support value}{\supportlower}{\supportlower}
    \macrorow{Upper support value}{\supportupper}{\supportupper}
    \macrorow{Certified-valid pairs}{\certvalid}{\certvalid}
    \macrorow{Certified-invalid pairs}{\certinvalid}{\certinvalid}
    \macrorow{Undecided pairs}{\undecided}{\undecided}
    \macrorow{Undecided rank}{\undecidedrank{\versionstate}}{\undecidedrank{\versionstate}}
    \macrorow{Randomized Markov policies}{\markovpolicies}{\markovpolicies}
    \macrorow{Markov residual uncertainty}{\bestversion}{\bestversion}
    \macrorow{Minimum undecided-reach probability}{\minreachprob}{\minreachprob}
    \macrorow{Undecided-hitting time}{\undecidedhittingtime}{\undecidedhittingtime}
    \macrorow{Episode filtration}{\episodicfiltration}{\episodicfiltration}
    \macrorow{Within-episode history}{\withinhistory}{\withinhistory}
    \macrorow{Sign pattern}{\signpattern}{\signpattern}
    \macrorow{Cells operator}{\cells}{\cells}
    \macrorow{Optimistic gate}{\optimisticgate}{\optimisticgate}
    \macrorow{Optimistic value}{\optimisticvalue}{\optimisticvalue}
    \macrorow{Optimistic action-value}{\optimisticq}{\optimisticq}
    \macrorow{Absorption event}{\absorptionevent}{\absorptionevent}
    \macrorow{Probing mistake}{\probingmistake}{\probingmistake}
    \macrorow{Cumulative regret}{\cumulativeregret}{\cumulativeregret}

    \macrotablesection{Routes, prices, potentials and probes}
    \macrorow{Route (within-episode policy)}{\route}{\route}
    \macrorow{Set of routes}{\routes}{\routes}
    \macrorow{Abort action (AB)}{\abortaction}{\abortaction}
    \macrorow{Undecided span}{\undecidedspan}{\undecidedspan}
    \macrorow{Undecided potential}{\undecidedpotential{\versionstate}}{\undecidedpotential{\versionstate}}
    \macrorow{Potential}{\potential}{\potential}
    \macrorow{Efficiency coefficient}{\efficiencycoef_{\potential}}{\efficiencycoef_{\potential}}
    \macrorow{Price of identification}{\price}{\price}
    \macrorow{Bellman operator on prices}{\priceoperator}{\priceoperator}
    \macrorow{Stopping episode}{\stoppingepisode}{\stoppingepisode}
    \macrorow{Adequacy certificate}{\certificate}{\certificate}
    \macrorow{Certified value}{\pessimisticvalue}{\pessimisticvalue}
    \macrorow{Certified actions}{\certifiedactions}{\certifiedactions}
    \macrorow{Certified model}{\certifiedmodel}{\certifiedmodel}
    \macrorow{Certified policy}{\certifiedpolicy}{\certifiedpolicy}
    \macrorow{Collected reward}{\collected}{\collected}
    \macrorow{Bonus program value}{\bonusvalue^{\lambda}}{\bonusvalue^{\lambda}}
    \macrorow{Continuation value}{\continuationvalue^{\lambda}}{\continuationvalue^{\lambda}}
    \macrorow{Certified price}{\certprice}{\certprice}
    \macrorow{Optimistic price}{\optprice}{\optprice}
    \macrorow{Optimistic shortfall}{\optshortfall}{\optshortfall}
    \macrorow{Target (undecided)}{\target_t(v)}{\target_t(v)}
    \macrorow{Aliased class (informative)}{\aliasedclass_{\versionstate}(v)}{\aliasedclass_{\versionstate}(v)}
    \macrorow{Informative pairs}{\informative}{\informative}
    \macrorow{Static instance-dependent bound}{\staticbound}{\staticbound}
    \macrorow{Cell value}{\cellvalue_{\gamma}}{\cellvalue_{\gamma}}
    \macrorow{Optimistic rivals}{\rivals}{\rivals}
    \macrorow{Falsification complexity}{\falscomplexity}{\falscomplexity}
    \macrorow{Realizable ceiling}{\cellvalue_{\versionstate}}{\cellvalue_{\versionstate}}
    \macrorow{Realizable price}{\realprice}{\realprice}
    \macrorow{Realizable certificate}{\realcertificate}{\realcertificate}
    \macrorow{Realizable shortfall}{\realshortfall}{\realshortfall}
    \macrorow{Cell policy}{\cellpolicy}{\cellpolicy}
    \macrorow{Refutation probability}{\refutationprob}{\refutationprob}
    \macrorow{Value loss of a cell}{\valueloss_{\maskpar}(\gamma)}{\valueloss_{\maskpar}(\gamma)}
    \macrorow{Harmonic number}{\harmonic{d}}{\harmonic{d}}

    \macrotablesection{Tasks and transfer}
    \macrorow{Task index}{\episode}{\episode}
    \macrorow{Number of tasks}{\episodes}{\episodes}
    \macrorow{Task data}{\dataset}{\dataset}
    \macrorow{History}{\history}{\history}
    \macrorow{Filtration}{\filtration}{\filtration}
    \macrorow{Confidence set}{\confset}{\confset}
    \macrorow{Backward-compatible set}{\compatset}{\compatset}
    \macrorow{Transfer input}{\transferinput}{\transferinput}
    \macrorow{Algorithm class}{\algorithmclass}{\algorithmclass}
    \macrorow{Task algorithm}{\taskalgorithm}{\taskalgorithm}
    \macrorow{Meta-policy}{\metapolicy}{\metapolicy}

    \macrotablesection{Matrix notation}
    \macrorow{Feature matrix}{\featurematrix}{\featurematrix}
    \macrorow{State feature matrix}{\statefeaturematrix{\state}}{\statefeaturematrix{\state}}
    \macrorow{Transition-feature matrix}{\transitionfeaturematrix}{\transitionfeaturematrix}
    \macrorow{Mask matrix}{\maskmatrix}{\maskmatrix}
    \macrorow{Policy matrix}{\policymatrix}{\policymatrix}
    \macrorow{Surviving transition kernel}{\survivalkernel}{\survivalkernel}
    \macrorow{Projection}{\projection}{\projection}

    \macrotablesection{Algorithm labels}
    \macrorow{First algorithm name}{\namealgone}{\text{\namealgone}}
    \macrorow{Second algorithm name}{\namealgtwo}{\text{\namealgtwo}}
  \end{longtable}
  \endgroup
}
